Privacy Protection, Measurement Error, and the Integration of Remote Sensing and Socioeconomic Survey Data

When publishing socioeconomic survey data, survey programs implement a variety of statistical methods designed to preserve privacy but which come at the cost of distorting the data. We explore the extent to which spatial anonymization methods to preserve privacy in the large-scale surveys supported by the World Bank Living Standards Measurement Study - Integrated Surveys on Agriculture (LSMS-ISA) introduce measurement error in econometric estimates when that survey data is integrated with remote sensing weather data. Guided by a pre-analysis plan, we produce 90 linked weather-household datasets that vary by the spatial anonymization method and the remote sensing weather product. By varying the data along with the econometric model we quantify the magnitude and significance of measurement error coming from the loss of accuracy that results from protect privacy measures. We find that spatial anonymization techniques currently in general use have, on average, limited to no impact on estimates of the relationship between weather and agricultural productivity. However, the degree to which spatial anonymization introduces mismeasurement is a function of which remote sensing weather product is used in the analysis. We conclude that care must be taken in choosing a remote sensing weather product when looking to integrate it with publicly available survey data.

==> tables/sumtab.tex <==
                    &\multicolumn{1}{c}{Ethiopia}&\multicolumn{1}{c}{Malawi}&\multicolumn{1}{c}{Niger}&\multicolumn{1}{c}{Nigeria}&\multicolumn{1}{c}{Tanzania}&\multicolumn{1}{c}{Uganda}\\
\midrule
\multicolumn{7}{l}{\emph{\textbf{Panel A}: Total Farm Production}}&            &            &            &            &            &            \\
Total farm production (2010 USD)&       245.4&       351.2&       188.5&       663.5&       207.3&       169.0\\
                    &     (322.8)&     (727.5)&     (201.7)&     (704.1)&     (269.4)&     (226.0)\\
Total farmed area (ha)&       1.055&       0.719&       11.14&       2.197&       1.598&       5.553\\
                    &     (5.670)&     (0.659)&     (15.59)&     (3.598)&     (2.985)&     (12.32)\\
Total farm yield (2010 USD/ha)&       440.6&       525.4&       60.93&       680.9&       235.2&       93.64\\
                    &     (607.2)&     (560.3)&     (169.0)&     (850.7)&     (286.8)&     (145.0)\\
Total farm labor rate (days/ha)&       434.4&       247.8&       94.94&       156.3&       311.1&       282.6\\
                    &     (834.9)&     (193.2)&     (219.1)&     (210.3)&     (353.9)&     (353.4)\\
Total farm fertilizer rate (kg/ha)&       56.26&       0.691&       5.120&       99.02&       20.89&       0.160\\
                    &     (94.98)&     (0.393)&     (23.83)&     (219.4)&     (68.17)&     (1.136)\\
Total farm pesticide use (\%)&      0.0615&      0.0418&      0.0800&       0.212&      0.0325&      0.0659\\
                    &     (0.240)&     (0.200)&     (0.271)&     (0.408)&     (0.177)&     (0.248)\\
Total farm herbicide use (\%)&       0.235&      0.0126&      0.0373&       0.292&      0.0981&      0.0295\\
                    &     (0.424)&     (0.112)&     (0.190)&     (0.455)&     (0.297)&     (0.169)\\
Total farm irrigation use (\%)&      0.0681&      0.0154&           0&      0.0270&      0.0422&      0.0202\\
                    &     (0.252)&     (0.123)&         (0)&     (0.162)&     (0.201)&     (0.141)\\
\midrule
\midrule Observations&        7272&        3250&        3913&        8384&        5669&        5250\\
\midrule
\multicolumn{7}{l}{\emph{\textbf{Panel B}: Primary Crop Production}}&            &            &            &            &            &            \\
Primary crop production (kg)&       314.6&       636.8&       471.5&       763.8&       608.5&       51.50\\
                    &     (476.6)&    (1035.3)&     (488.6)&    (1151.1)&     (793.5)&     (88.16)\\
Primary crop farmed area (ha)&       0.322&       0.661&       4.930&       0.720&       0.934&       1.501\\
                    &     (1.310)&     (0.622)&     (6.451)&     (1.115)&     (1.417)&     (2.669)\\
Primary crop yield (kg/ha)&      1593.2&      1191.8&       219.8&      1619.5&      1059.3&       87.89\\
                    &    (1782.8)&    (1242.1)&     (363.5)&    (2241.5)&    (1192.7)&     (146.7)\\
labor rate for maize (days/ha)&       466.1&       249.6&       70.72&       161.8&       263.2&       306.4\\
                    &     (666.6)&     (198.8)&     (121.1)&     (235.9)&     (295.9)&     (387.4)\\
Primary crop labor rate (days/ha)&       71.28&       0.722&       1.945&       146.3&       25.75&       0.196\\
                    &     (133.7)&     (0.399)&     (7.754)&     (302.0)&     (80.67)&     (1.638)\\
Primary crop pesticide use (\%)&      0.0259&      0.0388&      0.0550&       0.189&      0.0196&      0.0335\\
                    &     (0.159)&     (0.193)&     (0.228)&     (0.392)&     (0.139)&     (0.180)\\
Primary crop herbicide use (\%)&      0.0422&      0.0113&      0.0278&       0.378&      0.0945&      0.0219\\
                    &     (0.201)&     (0.106)&     (0.164)&     (0.485)&     (0.292)&     (0.146)\\
Primary crop irrigation use (\%)&      0.0515&      0.0141&           0&      0.0187&      0.0265&      0.0195\\
                    &     (0.221)&     (0.118)&         (0)&     (0.135)&     (0.161)&     (0.138)\\
\midrule
\midrule Observations&        3906&        3198&        3492&        3590&        4076&        2509\\


==> tables/var_sig_eth_rf.tex <==
                    &\multicolumn{1}{c}{CHIRPS}&\multicolumn{1}{c}{CPC}&\multicolumn{1}{c}{MERRA-2}&\multicolumn{1}{c}{ARC2}&\multicolumn{1}{c}{ERA5}&\multicolumn{1}{c}{TAMSAT}\\
\midrule
Mean Daily Rainfall &        0.58&        0.67&        0.67&        0.50&        0.83&        0.50\\
Median Daily Rainfall&        0.08&        0.83&        0.58&        0.25&        0.42&        0.50\\
Variance of Daily Rainfall&        0.58&        0.42&        0.58&        0.50&        0.67&        0.42\\
Skew of Daily Rainfall&        0.58&        0.50&        0.58&        0.75&        0.17&        0.25\\
Total Rainfall      &        0.58&        0.67&        0.67&        0.50&        0.83&        0.50\\
Deviation in Total Rainfall&        0.25&        0.58&        0.83&        0.00&        0.75&        0.17\\
Z-Score of Total Rainfall&        0.17&        0.42&        0.50&        0.17&        0.92&        0.25\\
Rainy Days          &        0.75&        0.67&        0.25&        0.83&        0.83&        0.92\\
Deviation in Rainy Days&        0.25&        0.58&        0.17&        0.42&        0.50&        0.83\\
No Rain Days        &        0.75&        0.33&        0.33&        0.83&        0.50&        0.75\\
Deviation in No Rain Days&        0.25&        0.58&        0.17&        0.42&        0.50&        0.83\\
\% Rainy Days       &        0.75&        0.67&        0.25&        0.83&        0.83&        0.92\\
Deviation in \% Rainy Days&        0.25&        0.58&        0.17&        0.42&        0.50&        0.83\\
Longest Dry Spell   &        0.33&        0.67&        0.42&        0.50&        0.42&        0.25\\
\midrule
Observations        &         168&         168&         168&         168&         168&         168\\


==> tables/var_sig_eth_tp.tex <==
                    &\multicolumn{1}{c}{MERRA-2}&\multicolumn{1}{c}{ERA5}&\multicolumn{1}{c}{CPC}\\
\midrule
Mean Daily Temperature&        0.67&        0.75&        0.50\\
Median Daily Temperature&        0.67&        0.58&        0.50\\
Variance of Daily Temperature&        0.33&        0.58&        0.50\\
Skew of Daily Temperature&        0.58&        0.25&        0.67\\
Growing Degree Days (GDD)&        0.17&        0.08&        0.33\\
Deviation in GDD    &        0.08&        0.25&        0.33\\
Z-Score of GDD      &        0.17&        0.25&        0.33\\
Maximum Daily Temperature&        0.33&        0.42&        0.42\\
\midrule
Observations        &          96&          96&          96\\


==> tables/var_sig_mwi_rf.tex <==
                    &\multicolumn{1}{c}{CHIRPS}&\multicolumn{1}{c}{CPC}&\multicolumn{1}{c}{MERRA-2}&\multicolumn{1}{c}{ARC2}&\multicolumn{1}{c}{ERA5}&\multicolumn{1}{c}{TAMSAT}\\
\midrule
Mean Daily Rainfall &        0.75&        0.67&        0.33&        0.67&        0.67&        0.75\\
Median Daily Rainfall&        0.17&        0.42&        0.92&        0.42&        0.50&        0.58\\
Variance of Daily Rainfall&        0.33&        0.33&        0.42&        0.17&        0.25&        0.33\\
Skew of Daily Rainfall&        0.92&        1.00&        0.42&        0.67&        0.08&        0.58\\
Total Rainfall      &        0.75&        0.67&        0.42&        0.67&        0.67&        0.75\\
Deviation in Total Rainfall&        0.17&        0.50&        0.33&        0.25&        0.67&        0.33\\
Z-Score of Total Rainfall&        0.25&        0.42&        0.33&        0.25&        0.33&        0.17\\
Rainy Days          &        0.67&        0.58&        0.42&        0.50&        0.42&        0.50\\
Deviation in Rainy Days&        0.75&        0.50&        0.67&        0.33&        0.58&        0.25\\
No Rain Days        &        0.67&        0.58&        0.42&        0.50&        0.50&        0.50\\
Deviation in No Rain Days&        0.75&        0.42&        0.67&        0.33&        0.58&        0.25\\
\% Rainy Days       &        0.67&        0.58&        0.42&        0.50&        0.42&        0.50\\
Deviation in \% Rainy Days&        0.75&        0.42&        0.67&        0.25&        0.58&        0.25\\
Longest Dry Spell   &        0.92&        0.58&        0.33&        0.58&        0.58&        0.25\\
\midrule
Observations        &         168&         168&         168&         168&         168&         168\\


==> tables/var_sig_mwi_tp.tex <==
                    &\multicolumn{1}{c}{MERRA-2}&\multicolumn{1}{c}{ERA5}&\multicolumn{1}{c}{CPC}\\
\midrule
Mean Daily Temperature&        0.92&        0.83&        0.67\\
Median Daily Temperature&        0.75&        0.83&        0.83\\
Variance of Daily Temperature&        0.50&        0.42&        0.58\\
Skew of Daily Temperature&        0.17&        0.25&        0.67\\
Growing Degree Days (GDD)&        0.83&        0.33&        0.42\\
Deviation in GDD    &        0.58&        0.42&        0.33\\
Z-Score of GDD      &        0.58&        0.58&        0.42\\
Maximum Daily Temperature&        0.58&        0.67&        0.67\\
\midrule
Observations        &          96&          96&          96\\


==> tables/var_sig_nga_rf.tex <==
                    &\multicolumn{1}{c}{CHIRPS}&\multicolumn{1}{c}{CPC}&\multicolumn{1}{c}{MERRA-2}&\multicolumn{1}{c}{ARC2}&\multicolumn{1}{c}{ERA5}&\multicolumn{1}{c}{TAMSAT}\\
\midrule
Mean Daily Rainfall &        0.58&        0.42&        0.58&        0.50&        0.83&        0.50\\
Median Daily Rainfall&        0.58&        0.33&        0.58&        0.58&        1.00&        0.58\\
Variance of Daily Rainfall&        0.75&        0.50&        0.25&        0.58&        0.83&        0.58\\
Skew of Daily Rainfall&        0.67&        0.42&        0.33&        0.42&        0.17&        0.42\\
Total Rainfall      &        0.58&        0.33&        0.67&        0.42&        0.83&        0.58\\
Deviation in Total Rainfall&        0.67&        0.50&        0.33&        0.50&        1.00&        0.50\\
Z-Score of Total Rainfall&        0.67&        0.92&        0.33&        0.17&        1.00&        0.67\\
Rainy Days          &        0.67&        0.50&        0.75&        0.67&        0.33&        0.75\\
Deviation in Rainy Days&        0.50&        0.58&        0.50&        0.58&        0.58&        0.58\\
No Rain Days        &        0.50&        0.42&        0.67&        0.42&        0.33&        0.58\\
Deviation in No Rain Days&        0.50&        0.58&        0.50&        0.58&        0.58&        0.58\\
\% Rainy Days       &        0.83&        0.58&        0.75&        0.83&        0.33&        0.92\\
Deviation in \% Rainy Days&        0.42&        0.75&        0.50&        0.33&        0.67&        0.58\\
Longest Dry Spell   &        0.42&        0.58&        0.33&        0.25&        0.58&        0.50\\
\midrule
Observations        &         168&         168&         168&         168&         168&         168\\


==> tables/var_sig_nga_tp.tex <==
                    &\multicolumn{1}{c}{MERRA-2}&\multicolumn{1}{c}{ERA5}&\multicolumn{1}{c}{CPC}\\
\midrule
Mean Daily Temperature&        0.58&        0.67&        0.58\\
Median Daily Temperature&        0.67&        0.75&        0.67\\
Variance of Daily Temperature&        0.75&        0.83&        0.58\\
Skew of Daily Temperature&        0.50&        0.42&        0.33\\
Growing Degree Days (GDD)&        0.75&        0.92&        0.83\\
Deviation in GDD    &        0.67&        0.67&        0.83\\
Z-Score of GDD      &        0.67&        0.83&        0.67\\
Maximum Daily Temperature&        0.67&        0.58&        0.58\\
\midrule
Observations        &          96&          96&          96\\


==> tables/var_sig_ngr_rf.tex <==
                    &\multicolumn{1}{c}{CHIRPS}&\multicolumn{1}{c}{CPC}&\multicolumn{1}{c}{MERRA-2}&\multicolumn{1}{c}{ARC2}&\multicolumn{1}{c}{ERA5}&\multicolumn{1}{c}{TAMSAT}\\
\midrule
Mean Daily Rainfall &        0.67&        0.67&        0.42&        0.67&        0.83&        0.33\\
Median Daily Rainfall&        0.00&        0.00&        0.58&        0.00&        0.00&        0.58\\
Variance of Daily Rainfall&        0.75&        0.83&        0.50&        0.67&        0.58&        0.25\\
Skew of Daily Rainfall&        0.42&        0.33&        0.42&        0.42&        0.42&        0.33\\
Total Rainfall      &        0.67&        0.67&        0.42&        0.67&        0.83&        0.33\\
Deviation in Total Rainfall&        0.58&        0.92&        0.83&        0.67&        0.67&        0.25\\
Z-Score of Total Rainfall&        0.58&        0.83&        0.83&        0.67&        0.50&        0.17\\
Rainy Days          &        0.42&        0.42&        0.58&        0.75&        0.67&        0.67\\
Deviation in Rainy Days&        0.58&        0.42&        0.50&        0.25&        0.00&        0.67\\
No Rain Days        &        0.50&        0.33&        0.58&        0.67&        0.58&        0.67\\
Deviation in No Rain Days&        0.58&        0.42&        0.50&        0.25&        0.00&        0.67\\
\% Rainy Days       &        0.42&        0.42&        0.58&        0.75&        0.67&        0.67\\
Deviation in \% Rainy Days&        0.58&        0.42&        0.50&        0.25&        0.00&        0.67\\
Longest Dry Spell   &        0.58&        0.75&        0.75&        0.42&        0.58&        0.75\\
\midrule
Observations        &         168&         168&         168&         168&         168&         168\\


==> tables/var_sig_ngr_tp.tex <==
                    &\multicolumn{1}{c}{MERRA-2}&\multicolumn{1}{c}{ERA5}&\multicolumn{1}{c}{CPC}\\
\midrule
Mean Daily Temperature&        0.50&        0.58&        0.58\\
Median Daily Temperature&        0.50&        0.67&        0.67\\
Variance of Daily Temperature&        0.50&        0.83&        0.50\\
Skew of Daily Temperature&        0.50&        0.50&        0.58\\
Growing Degree Days (GDD)&        0.50&        0.50&        0.75\\
Deviation in GDD    &        0.50&        0.50&        0.75\\
Z-Score of GDD      &        0.33&        0.67&        0.67\\
Maximum Daily Temperature&        0.83&        0.58&        0.83\\
\midrule
Observations        &          96&          96&          96\\


==> tables/var_sig_tza_rf.tex <==
                    &\multicolumn{1}{c}{CHIRPS}&\multicolumn{1}{c}{CPC}&\multicolumn{1}{c}{MERRA-2}&\multicolumn{1}{c}{ARC2}&\multicolumn{1}{c}{ERA5}&\multicolumn{1}{c}{TAMSAT}\\
\midrule
Mean Daily Rainfall &        0.33&        0.50&        0.50&        0.33&        0.42&        0.25\\
Median Daily Rainfall&        0.25&        0.08&        0.33&        0.25&        0.42&        0.25\\
Variance of Daily Rainfall&        0.25&        0.58&        0.58&        0.08&        0.25&        0.58\\
Skew of Daily Rainfall&        0.25&        0.50&        0.08&        0.42&        0.17&        0.25\\
Total Rainfall      &        0.33&        0.50&        0.50&        0.33&        0.42&        0.25\\
Deviation in Total Rainfall&        0.33&        0.33&        0.33&        0.17&        0.58&        0.17\\
Z-Score of Total Rainfall&        0.25&        0.50&        0.25&        0.17&        0.33&        0.17\\
Rainy Days          &        0.58&        0.58&        0.75&        0.50&        0.58&        0.42\\
Deviation in Rainy Days&        0.50&        0.42&        0.92&        0.33&        0.33&        0.33\\
No Rain Days        &        0.42&        0.75&        0.58&        0.50&        0.67&        0.33\\
Deviation in No Rain Days&        0.50&        0.42&        0.92&        0.33&        0.33&        0.33\\
\% Rainy Days       &        0.58&        0.58&        0.75&        0.50&        0.58&        0.42\\
Deviation in \% Rainy Days&        0.50&        0.42&        0.92&        0.33&        0.33&        0.33\\
Longest Dry Spell   &        0.08&        0.58&        0.17&        0.25&        0.25&        0.42\\
\midrule
Observations        &         168&         168&         168&         168&         168&         168\\


==> tables/var_sig_tza_tp.tex <==
                    &\multicolumn{1}{c}{MERRA-2}&\multicolumn{1}{c}{ERA5}&\multicolumn{1}{c}{CPC}\\
\midrule
Mean Daily Temperature&        0.50&        0.42&        0.33\\
Median Daily Temperature&        0.33&        0.58&        0.50\\
Variance of Daily Temperature&        0.67&        0.67&        0.58\\
Skew of Daily Temperature&        0.42&        0.33&        0.33\\
Growing Degree Days (GDD)&        0.00&        0.00&        0.67\\
Deviation in GDD    &        0.25&        0.00&        0.50\\
Z-Score of GDD      &        0.42&        0.00&        0.50\\
Maximum Daily Temperature&        0.33&        0.50&        0.42\\
\midrule
Observations        &          96&          96&          96\\


==> tables/var_sig_uga_rf.tex <==
                    &\multicolumn{1}{c}{CHIRPS}&\multicolumn{1}{c}{CPC}&\multicolumn{1}{c}{MERRA-2}&\multicolumn{1}{c}{ARC2}&\multicolumn{1}{c}{ERA5}&\multicolumn{1}{c}{TAMSAT}\\
\midrule
Mean Daily Rainfall &        0.33&        0.75&        0.58&        0.58&        0.58&        0.42\\
Median Daily Rainfall&        0.33&        0.08&        0.50&        0.33&        0.50&        0.50\\
Variance of Daily Rainfall&        0.42&        0.75&        0.67&        0.50&        0.67&        0.33\\
Skew of Daily Rainfall&        0.33&        0.42&        0.42&        0.17&        0.42&        0.50\\
Total Rainfall      &        0.33&        0.75&        0.67&        0.67&        0.58&        0.50\\
Deviation in Total Rainfall&        0.33&        0.58&        0.50&        0.58&        0.58&        0.58\\
Z-Score of Total Rainfall&        0.25&        0.42&        0.33&        0.58&        0.75&        0.58\\
Rainy Days          &        0.25&        0.58&        0.42&        0.50&        0.67&        0.67\\
Deviation in Rainy Days&        0.17&        0.33&        0.50&        0.58&        0.50&        0.67\\
No Rain Days        &        0.25&        0.58&        0.42&        0.42&        0.50&        0.67\\
Deviation in No Rain Days&        0.17&        0.42&        0.50&        0.58&        0.58&        0.67\\
\% Rainy Days       &        0.25&        0.58&        0.42&        0.42&        0.67&        0.67\\
Deviation in \% Rainy Days&        0.17&        0.33&        0.50&        0.58&        0.58&        0.67\\
Longest Dry Spell   &        0.50&        0.33&        0.50&        0.42&        0.58&        0.33\\
\midrule
Observations        &         168&         168&         168&         168&         168&         168\\


==> tables/var_sig_uga_tp.tex <==
                    &\multicolumn{1}{c}{MERRA-2}&\multicolumn{1}{c}{ERA5}&\multicolumn{1}{c}{CPC}\\
\midrule
Mean Daily Temperature&        0.58&        0.58&        0.42\\
Median Daily Temperature&        0.58&        0.58&        0.58\\
Variance of Daily Temperature&        0.42&        0.50&        0.17\\
Skew of Daily Temperature&        0.50&        0.50&        0.33\\
Growing Degree Days (GDD)&        0.25&        0.50&        0.50\\
Deviation in GDD    &        0.33&        0.67&        0.17\\
Z-Score of GDD      &        0.33&        0.33&        0.42\\
Maximum Daily Temperature&        0.50&        0.25&        0.67\\
\midrule
Observations        &          96&          96&          96\\


==> tables/var_sum_cp.tex <==
                    &\multicolumn{1}{c}{Ethiopia}&\multicolumn{1}{c}{Malawi}&\multicolumn{1}{c}{Niger}&\multicolumn{1}{c}{Nigeria}&\multicolumn{1}{c}{Tanzania}&\multicolumn{1}{c}{Uganda}\\
\midrule
Primary crop production (kg)&     314.628&     636.821&     471.515&     763.775&     608.486&      51.501\\
                    &   (476.561)&  (1035.265)&   (488.566)&  (1151.052)&   (793.543)&    (88.163)\\
Primary crop farmed area (ha)&       0.322&       0.661&       4.930&       0.720&       0.934&       1.501\\
                    &     (1.310)&     (0.622)&     (6.451)&     (1.115)&     (1.417)&     (2.669)\\
Primary crop yield (kg/ha)&    1593.185&    1191.798&     219.831&    1619.457&    1059.326&      87.887\\
                    &  (1782.828)&  (1242.061)&   (363.483)&  (2241.451)&  (1192.715)&   (146.689)\\
Primary crop labor rate (days/ha)&     466.074&     249.630&      70.716&     161.817&     263.232&     306.384\\
                    &   (666.579)&   (198.766)&   (121.063)&   (235.852)&   (295.932)&   (387.407)\\
Primary crop fertilizer rate (kg/ha)&      71.278&       0.722&       1.945&     146.287&      25.753&       0.196\\
                    &   (133.675)&     (0.399)&     (7.754)&   (302.022)&    (80.668)&     (1.638)\\
Primary crop pesticide use (\%)&       0.026&       0.039&       0.055&       0.189&       0.020&       0.033\\
                    &     (0.159)&     (0.193)&     (0.228)&     (0.392)&     (0.139)&     (0.180)\\
Primary crop herbicide use (\%)&       0.042&       0.011&       0.028&       0.378&       0.094&       0.022\\
                    &     (0.201)&     (0.106)&     (0.164)&     (0.485)&     (0.292)&     (0.146)\\
Primary crop irrigation use (\%)&       0.051&       0.014&       0.000&       0.019&       0.026&       0.020\\
                    &     (0.221)&     (0.118)&     (0.000)&     (0.135)&     (0.161)&     (0.138)\\
\midrule
Observations        &        3906&        3198&        3492&        3590&        4076&        2509\\


==> tables/var_sum_tf.tex <==
                    &\multicolumn{1}{c}{Ethiopia}&\multicolumn{1}{c}{Malawi}&\multicolumn{1}{c}{Niger}&\multicolumn{1}{c}{Nigeria}&\multicolumn{1}{c}{Tanzania}&\multicolumn{1}{c}{Uganda}\\
\midrule
Total farm production (2010 USD)&     245.443&     351.200&     188.483&     663.534&     207.253&     168.963\\
                    &   (322.836)&   (727.512)&   (201.741)&   (704.067)&   (269.391)&   (226.006)\\
Total farmed area (ha)&       1.055&       0.719&      11.144&       2.197&       1.598&       5.553\\
                    &     (5.670)&     (0.659)&    (15.591)&     (3.598)&     (2.985)&    (12.319)\\
Total farm yield (2010 USD/ha)&     440.563&     525.363&      60.931&     680.936&     235.204&      93.638\\
                    &   (607.222)&   (560.263)&   (169.031)&   (850.662)&   (286.760)&   (145.023)\\
Total farm labor rate (days/ha)&     434.411&     247.781&      94.944&     156.287&     311.122&     282.568\\
                    &   (834.853)&   (193.168)&   (219.098)&   (210.296)&   (353.920)&   (353.363)\\
Total farm fertilizer rate (kg/ha)&      56.260&       0.691&       5.120&      99.021&      20.890&       0.160\\
                    &    (94.979)&     (0.393)&    (23.833)&   (219.442)&    (68.174)&     (1.136)\\
Total farm pesticide use (\%)&       0.061&       0.042&       0.080&       0.212&       0.032&       0.066\\
                    &     (0.240)&     (0.200)&     (0.271)&     (0.408)&     (0.177)&     (0.248)\\
Total farm herbicide use (\%)&       0.235&       0.013&       0.037&       0.292&       0.098&       0.030\\
                    &     (0.424)&     (0.112)&     (0.190)&     (0.455)&     (0.297)&     (0.169)\\
Total farm irrigation use (\%)&       0.068&       0.015&       0.000&       0.027&       0.042&       0.020\\
                    &     (0.252)&     (0.123)&     (0.000)&     (0.162)&     (0.201)&     (0.141)\\
\midrule
Observations        &        7272&        3250&        3913&        8384&        5669&        5250\\

